Multi-Objective Reward and Preference Optimization: Theory and Algorithms

This thesis develops theoretical frameworks and algorithms that advance constrained reinforcement learning (RL) across control, preference learning, and alignment of large language models. The first contribution addresses constrained Markov Decision Processes (CMDPs) under the average-cost criterion through the Average-Constrained Policy Optimization (ACPO) algorithm. ACPO integrates sensitivity analysis with trust-region updates to ensure stable constraint handling, achieving state-of-the-art empirical performance with theoretical guarantees. Constrained RL is then extended to finite-horizon settings via e-COP, the first policy optimization method for episodic CMDPs. Built on an episodic policy difference lemma, e-COP offers provable performance, simplicity, and scalability in safety-critical environments. The thesis then investigates reinforcement learning from human preferences. warmPref-PS introduces a posterior sampling strategy for linear bandits that integrates offline preference data from heterogeneous raters into online learning. Explicit modeling of rater competence yields substantial regret reduction and more efficient data collection for RLHF. The PSPL algorithm further advances preference-based RL by jointly sampling reward models and transition dynamics from pairwise trajectory comparisons, providing Bayesian simple-regret guarantees and robust empirical identification of optimal policies. The final contribution applies these methods to large-scale model alignment. A multi-objective constrained optimization view yields MOPO, an iterative algorithm with closed-form updates that scales to multi-billion-parameter language models and remains robust across alignment settings. Collectively, the thesis unifies constrained RL across average-cost, episodic, and preference-driven paradigms, delivering theoretical advances and practical tools for safe and aligned decision-making.

==> chapter2/conclusion.tex <==
\section{Conclusion}
\label{sec:conclusion}

In this chapter, we have introduced an easy to implement, scalable policy optimization algorithm for episodic RL problems with constraints due to safety or other considerations. It is based on a policy difference lemma for the episodic setting, which surprisingly has quite a different form than the ones for infinite-horizon discounted or average settings. This provides the theoretical foundation for the algorithm, which is designed by incorporating several time-tested, practical as well as novel ideas. Policy optimization algorithms for Constrained MDPs tend to be numerical unstable and non-scalable due to the need for inverting the Fisher information matrix. We sidestep both of these issues by introducing a quadratic damping penalty term that works remarkably well. The algorithm development is well supported by theory, as well as with extensive empirical analysis on a range of Safety Gym and Safe MuJoco benchmark environments against a suite of baseline algorithms adapted from their non-episodic roots. 
% The development here is partly motivated by the need for practical and scalable episodic constrained policy optimization algorithms for fine-tuning image diffusion and large language models so that they generate safe outputs at inference time.

%In this work, we introduced Episodic Constrained Optimization for Policies (e-COP), a novel quadratic-penalty based policy optimization algorithm aimed at solving episodic CMDPs. We emphasize the need for separate theory and algorithmic design for episodic RL, as existing algorithms tailored for infinite horizon discounted settings may result in performance degradation. We first introduce the principled approach of using a policy optimization algorithm in episodic setting, and further develop it to introduce e-COP. We provide both theoretical and empirical results supporting the advantages of e-COP, including ease of implementation, stable convergence without oscillation, and precise penalty application to prevent suboptimal policies. e-COP outperforms current state-of-the-art safe RL baselines across a variety of tasks in the episodic setting. Looking ahead, we aim to explore the application of episodic RL in tasks such as image diffusion and safety-layer optimization in large language models.


==> chapter3/conclusion.tex <==
\section{Conclusion}
\label{sec:chapter3_conclusion}

In this paper, we proposed $\mathsf{warmPref-PS}$, a Bayesian posterior sampling-based algorithm that efficiently incorporates offline preference data to warm-start the online learning phase. We provide theoretical foundations for bridging the gap between fixed, offline preferences and online learning. 
% To this extent, we provide bounds on the size of offline dataset needed to infer the optimal action, while minimizing Bayesian regret simultaneously. 
We further introduced Bootstrapped $\mathsf{warmPref-PS}$, a computationally tractable extension designed to handle large-scale environments. Our theoretical results and empirical evaluations demonstrate the robustness and superior performance of $\mathsf{warmPref-PS}$. While additional work is needed to refine our approach for RLHF, we provide a promising foundation for further development in this space.



%In this work, we have delved into the procedure of integrating offline preferences to improve online learning. While it's intuitive to anticipate improved performance with an offline dataset, our investigation delves deeper into the mechanisms and degree of this improvement. Motivated by our experimental findings, we demonstrate that employing the preferences in a straightforward manner yields only marginal reductions in regret. However, adopting a more sophisticated approach, which incorporates considerations of expert competence levels can lead to significant reductions in cumulative regret. Since the goal of our work is to yield insights on how to usethe offline preferences to improve online learning, we have used a prototypical finite linear multi-armed bandits learning model, and a mathematically straightforward expert policy. However, it's worth noting the potential for application in more complex environments and models, such as MDPs, pretraining of LLMs, and broader generative models of expert policies. We aim to investigate these settings in future work.

==> chapter4/conclusion.tex <==

\section{Conclusion}
\label{sec:pspl_conclusion}

We have proposed the $\PSPL$ algorithm that incorporates offline preferences to learn an MDP with unknown rewards and transitions. We provide the first analysis to bridge the gap between offline preferences and online learning. We also introduced Bootstrapped $\PSPL$, a computationally tractable extension, and our empirical results demonstrate superior performance of $\PSPL$ in challenging benchmarks as compared to baselines. Overall, we provide a promising foundation for further development in PbRL and RLHF space.



==> specs/abstract.tex <==
% the abstract

Reinforcement learning (RL) is a machine learning (ML) technique on learning to make optimal
sequential decisions via interactions with an environment. In recent years, RL has achieved great success in many artificial intelligence tasks, and has been widely regarded as one of the keys towards Artificial General Intelligence (AGI). Through this, constrained RL has emerged as a critical area of study, addressing the challenges of optimizing behavior under constraints across diverse application domains. This thesis develops novel theoretical foundations and practical algorithms to advance the field of constrained RL.

The thesis begins by tackling the problem of constrained Markov Decision Processes (CMDPs) under the average criterion, introducing the Average-Constrained Policy Optimization (ACPO) algorithm. By leveraging sensitivity theory and trust-region optimization techniques, ACPO delivers superior empirical performance and provides strong theoretical guarantees, outperforming state-of-the-art approaches in complex environments. Next, the constrained RL setting is extended to episodic settings with the development of the \texttt{e-COP} algorithm, the first policy optimization framework specifically tailored for finite-horizon CMDPs. Grounded in a novel policy difference lemma for episodic settings, \texttt{e-COP} combines simplicity, scalability, and robust theoretical guarantees. Its success in safety-constrained benchmarks highlights its potential for broader applications, such as in Reinforcement Learning from Human Feedback (RLHF).

To address the growing importance of RLHF in context of AGI, there is a need for methods to incorporate human preference feedback into RL algorithms. Recognizing the challenges posed by noisy human feedback, \texttt{warmPref-PS} is proposed, which is a posterior sampling algorithm designed to integrate offline preference data from raters of varying competence into online learning in a linear bandit environment. The algorithm achieves significant regret reduction and demonstrates the efficacy of modeling rater competence for adaptive data collection and fine-tuning in RLHF scenarios. Finally, a deep-dive into preference-based RL (PbRL), where learning is driven by binary trajectory comparisons rather than explicit rewards, is done. By leveraging offline datasets and modeling rater competence, the $\mathsf{PSPL}$ algorithm, which integrates posterior sampling for both reward models and transition dynamics, is presented. Theoretical Bayesian simple regret bounds for $\mathsf{PSPL}$ are established and empirical results demonstrate its correctness and robustness in identifying optimal policies.

Finally, we combine the above optimization and theoretical RLHF methodologies into practice. Multi-objective alignment of large language models is studied through the lens of constrained optimization, where a primary objective is maximized and secondary objectives are constrained to be above tunable thresholds. This results in an iterative algorithm, called \texttt{MOPO}, with closed-form updates, scalability to multi-billion parameter LLMs, and robustness to hyperparameters. 

Through these contributions, this thesis unifies constrained RL under diverse paradigms, from policy optimization to preference alignment, advancing both the theoretical understanding and practical efficacy of constrained decision-making.



==> specs/outro.tex <==
\newpage

% If you do want an image in the colophon:
% \begin{figure}
%   \vspace{50pt}
%   \centering
%     \includegraphics[width=0.95\textwidth]{images/cmu.jpeg}
% \end{figure}

% If you don't want an image in the colophon:
% \vspace*{200pt}

\begin{center}
\parbox{350pt}{\lettrine[lines=3,slope=-2pt,nindent=-4pt]{\textcolor{SchoolColor}{T}}{ his thesis was} researched for at Carnegie Mellon University under the grateful advisement of Professor Ding Zhao. The above picture was taken on 14\textsuperscript{th} November 2019 in the foyer of Carnegie Mellon's Tepper School of Business. It was my last day in Pittsburgh before I came back to India to finish my last semester of undergraduate life. I am, and will always be, very grateful to all the people who helped make this experience worthwhile.}
\end{center}
